Resilient Estimator-based Control Barrier Functions for Dynamical Systems with Disturbances and Noise

Control Barrier Function (CBF) is an emerging method that guarantees safety in path planning problems by generating a control command to ensure the forward invariance of a safety set. Most of the developments up to date assume availability of correct state measurements and absence of disturbances on the system. However, if the system incurs disturbances and is subject to noise, the CBF cannot guarantee safety due to the distorted state estimate. To improve the resilience and adaptability of the CBF, we propose a resilient estimator-based control barrier function (RE-CBF), which is based on a novel stochastic CBF optimization and resilient estimator, to guarantee the safety of systems with disturbances and noise in the path planning problems. The proposed algorithm uses the resilient estimation algorithm to estimate disturbances and counteract their effect using novel stochastic CBF optimization, providing safe control inputs for dynamical systems with disturbances and noise. To demonstrate the effectiveness of our algorithm in handling both noise and disturbances in dynamics and measurement, we design a quadrotor testing pipeline to simulate the proposed algorithm and then implement the algorithm on a real drone in our flying arena. Both simulations and real-world experiments show that the proposed method can guarantee safety for systems with disturbances and noise.

==> z_0_notes.tex <==
{\Blue

\section*{Deadlines}

\begin{itemize}
    % \item  \st{Indicating the interest: April 30, 2022;}
    %     \begin{itemize}
    %         \item \st{Tentative title of your paper along with a list of authors.}
    %         \item \st{Couple lines describing the main goal of your paper, not necessarily an abstract.}
    %     \end{itemize}
    % \item  \st{Extended abstract (>1000 words):  June 1, 2022;}
    \item conference website: \href{https://www.aiaa.org/SciTech/presentations-papers}{https://www.aiaa.org/SciTech/presentations-papers}
    % \item Author Notifications: Aug. 31, 2022 (accepted)
    \item  {\dred Paper submission: Dec. 5, 2022. }
    % \item \href{https://arxiv.org/pdf/2203.11470.pdf}{https://arxiv.org/pdf/2203.11470.pdf}
    \item \st{Drone implementation} [simulation only for the AIAA submission]
\end{itemize}

}

 
 
 
% {\dred
% \subsection*{Indicating the interest \hl{(Send to Naira by around April 29)}}

% {\textbf{Tentative title:}}

% Resilient Control Barrier Functions for Uncertain Systems

% \medskip

% \textbf{List of authors:}

% Chuyuan Tao, Wenbin Wan, Hunmin Kim, Pan Zhao, and Naira Hovakimyan
% }

% \medskip

% {\Blue
% \hl{\textbf{Couple lines describing the main goal:}}

% The control barrier function (CBF) is widely used to guarantee safety for autonomous systems, under the assumption that the state of the system is known and the dynamic system is fault-free. To enhance fault resiliency and adaptability, we will develop a resilient control barrier function framework for dynamic systems subject to biased and potentially large uncertainties by integrating the resilient estimation and control barrier functions. In this framework, the resilient estimation algorithm provides the size of biased uncertainties and quantifies uncertainties of the state estimates. We will use the quantified state estimation uncertainty in CBF to guarantee safety in the presence of measurement uncertainties. Furthermore, CBF will compensate for the estimated biased uncertainty to keep the desired performance. To ensure closed-loop stability, we will analyze the end-to-end stability of the whole framework.}

% =================================================================



% \medskip


% %

% \subsection*{Papers shared}
% \begin{itemize}
%     \item Control Barrier Functions for Stochastic Systems \url{https://arxiv.org/pdf/2003.03498.pdf}
    
%     \item Discrete Control Barrier Functions \url{http://www.roboticsproceedings.org/rss13/p73.pdf}
% \end{itemize}





% \newpage
